Uncovering the Benefits and Challenges of Continuous Integration Practices

In 2006, Fowler and Foemmel defined ten core Continuous Integration (CI) practices that could increase the speed of software development feedback cycles and improve software quality. Since then, these practices have been widely adopted by industry and subsequent research has shown they improve software quality. However, there is poor understanding of how organizations implement these practices, of the benefits developers perceive they bring, and of the challenges developers and organizations experience in implementing them. In this paper, we discuss a multiple-case study of three small- to medium-sized companies using the recommended suite of ten CI practices. Using interviews and activity log mining, we learned that these practices are broadly implemented but how they are implemented varies depending on their perceived benefits, the context of the project, and the CI tools used by the organization. We also discovered that CI practices can create new constraints on the software process that hurt feedback cycle time. For researchers, we show that how CI is implemented varies, and thus studying CI (for example, using data mining) requires understanding these differences as important context for research studies. For practitioners, our findings reveal in-depth insights on the possible benefits and challenges from using the ten practices, and how project context matters.

==> tbl_practices_themes.tex <==
\begin{table*}[!t]
	\caption{Themes reported by organizations per practice}
	\label{tbl:practices_themes}
	\centering
	\begin{tabularx}{2\columnwidth}{m{4cm} m{4cm} m{4cm} m{4cm}}
		\toprule[1pt]
		\textbf{Practice} & \textbf{ORG A} & \textbf{ORG B} & \textbf{ORG C} \\
		\toprule[1pt]
		% P1: Maintain a single source repository
		Maintain a single source repository &
		\begin{itemize}
			\item 
		\end{itemize} &
		\begin{itemize}
			\item 
		\end{itemize}  &
		\begin{itemize}
			\item 
		\end{itemize} \\
		\midrule
		% P2: Automate the build
		Automate the build &
		\begin{itemize}
			\item 
		\end{itemize} &
		\begin{itemize}
			\item 
		\end{itemize}  &
		\begin{itemize}
			\item Automation delegates repeatable tasks to a tool.
			\item Automation-induced velocity possibly mitigated by too many gates.
		\end{itemize} \\
		\midrule
		% P3: Make the build self-testing
		Make the build self-testing &
		\begin{itemize}
			\item 
		\end{itemize} &
		\begin{itemize}
			\item 
		\end{itemize}  &
		\begin{itemize}
			\item All types of tests are included in the build.
			\item Extensive testing increases build duration.
		\end{itemize} \\
		\midrule
		% P4: Everyone commits to the mainline every day
		Everyone commits to the mainline every day &
		\begin{itemize}
			\item 
		\end{itemize} &
		\begin{itemize}
			\item 
		\end{itemize}  &
		\begin{itemize}
			\item The combination of feature branches and large task sizes increases divergence from mainline.
		\end{itemize} \\
		\midrule
		% P5: Every commit should build the mainline on an integration machine
		Every commit should build the mainline on an integration machine &
		\begin{itemize}
			\item 
		\end{itemize} &
		\begin{itemize}
			\item 
		\end{itemize}  &
		\begin{itemize}
			\item To conserve resources, older builds in a concurrent pair are dropped in favor of newer ones.
		\end{itemize} \\
		\midrule
		% P6: Keep the build fast
		Keep the build fast &
		\begin{itemize}
			\item 
		\end{itemize} &
		\begin{itemize}
			\item 
		\end{itemize}  &
		\begin{itemize}
			\item Extensive testing increases build duration.
			\item Test execution strategy (serial) impacted by build infrastructure resource constraints.
		\end{itemize} \\
		\midrule
		% P7: Test in a clone of the production environment
		Test in a clone of the production environment &
		\begin{itemize}
			\item 
		\end{itemize} &
		\begin{itemize}
			\item 
		\end{itemize}  &
		\begin{itemize}
			\item It is infeasible to test a SaaS application in a complete production clone.
		\end{itemize} \\
		\midrule
		% P8: Make it easy for anyone to get the latest executable
		Make it easy for anyone to get the latest executable &
		\begin{itemize}
			\item 
		\end{itemize} &
		\begin{itemize}
			\item 
		\end{itemize}  &
		\begin{itemize}
			\item Build tools facilitate knowledge transfer -- useful for onboarding.
		\end{itemize} \\
		\midrule
		% P9: Ensure that system state and changes are visible:
		Ensure that system state and changes are visible &
		\begin{itemize}
			\item 
		\end{itemize} &
		\begin{itemize}
			\item 
		\end{itemize}  &
		\begin{itemize}
			\item Other teams have visibility into the development process.
		\end{itemize} \\
		\midrule
		% P10: Automate deployment
		Automate deployment &
		\begin{itemize}
			\item 
		\end{itemize} &
		\begin{itemize}
			\item 
		\end{itemize}  &
		\begin{itemize}
			\item Deployment frequency is heavily influenced by customer schedules.
			\item Deployments take a long time due to testing and drafting release notes.
		\end{itemize} \\
		\bottomrule[1pt]
	\end{tabularx}
\end{table*}
